Boardman-Vogt tensor product and wreath product of operadic categories

We introduce the wreath product of operadic categories and show that it produces a monoidal structure on the category OpCat of strict operadic categories. We relate the wreath product to the well known Boardman-Vogt tensor product of operads by interpreting the category of symmetric set-valued colored unital operads as a reflexive subcategory of OpCat. Our main result is that the reflection is a strong monoidal functor. In particular, the Boardman-Vogt tensor product of two colored operads in Set is isomorphic to an operad that is induced by the wreath product of suitable operadic categories.

==> interchange_intro.tex <==
\mytreesq[$\alpha$,$\beta$,bl,vert,$T_{1,1}$,$T_{1,k}$,$T_{j,1}$,$T_{j,k}$] ~~~=~~~ \mytreesq[$\beta$,$\alpha$,vert,bl,$T_{1,1}$,$T_{j,1}$,$T_{1,k}$,$T_{j,k}$].

==> interchange_prelim.tex <==
\tikz[baseline=.1ex]{
\tikzset{square/.style={regular polygon,regular polygon sides=4}}
\tikzset{bl/.style = {shape=ellipse,draw=black,inner sep=1.5pt}}
\tikzset{vert/.style = {shape=ellipse,draw=black,fill={gray!30},inner sep=1.5pt}}
    \node at (0,-1.5) (root) {$(c,d)$};
    \node [bl] (row1) at (0,-.5) {$x \otimes d$};
    \node (row1left) at (-1.6, -.2) {${(c_1,d)}$};
    \node (row1left) at (1.6, -.2) {${(c_n,d)}$};
    \node (dots1) at (0,.5) {$\cdots$};
    \node [vert] (row2_1) at (-2, .5) {$c_1 \otimes y$};
    \node [vert] (row2_2) at (2, .5) {$c_n \otimes y$};
    \node at (-2.9,1.5)  (row3_1) {${(c_1,d_1)}$};
    \node (dots1) at (-2,1.5) {$\cdots$};
    \node at (-1.1,1.5)  (row3_2) {${(c_1, d_m)}$};
    \node at (1.1,1.5)  (row3_3) {${(c_n, d_1)}$};
    \node (dots1) at (2,1.5) {$\cdots$};
    \node at (2.9,1.5)  (row3_4) {${(c_n,d_m)}$};

    \draw (root) -- (row1);
    \draw (row1) -- (row2_1);
    \draw (row1) -- (row2_2);
    \draw (row2_1) -- (row3_1);
    \draw (row2_1) -- (row3_2);
    \draw (row2_2) -- (row3_3);
    \draw (row2_2) -- (row3_4);
}
~~~$\mathlarger{\mathlarger{\mathlarger{\neq}}}$~~~ 
\tikz[baseline=.1ex]{
\tikzset{square/.style={regular polygon,regular polygon sides=4}}
\tikzset{bl/.style = {shape=ellipse,draw=black,inner sep=1.5pt}}
\tikzset{vert/.style = {shape=ellipse,draw=black,fill={gray!30},inner sep=1.5pt}}
    \node at (0,-1.5) (root) {$(c,d)$};
    \node [vert] (row1) at (0,-.5) {$c \otimes y$};
    \node (row1left) at (-1.6, -.2) {${(c,d_1)}$};
    \node (row1left) at (1.6, -.2) {${(c,d_m)}$};
    \node (dots1) at (0,.5) {$\cdots$};
    \node [bl] (row2_1) at (-2, .5) {$x \otimes d_1$};
    \node [bl] (row2_2) at (2, .5) {$x \otimes d_m$};
    \node at (-2.9,1.5)  (row3_1) {${(c_1, d_1)}$};
    \node (dots1) at (-2,1.5) {$\cdots$};
    \node at (-1.1,1.5)  (row3_2) {${(c_n, d_1)}$};
    \node at (1.1,1.5)  (row3_3) {${(c_1, d_m)}$};
    \node (dots1) at (2,1.5) {$\cdots$};
    \node at (2.9,1.5)  (row3_4) {$(c_n, d_m)$};

    \draw (root) -- (row1);
    \draw (row1) -- (row2_1);
    \draw (row1) -- (row2_2);
    \draw (row2_1) -- (row3_1);
    \draw (row2_1) -- (row3_2);
    \draw (row2_2) -- (row3_3);
    \draw (row2_2) -- (row3_4);
}


